CogSys: Efficient and Scalable Neurosymbolic Cognition System via Algorithm-Hardware Co-Design

Neurosymbolic AI is an emerging compositional paradigm that fuses neural learning with symbolic reasoning to enhance the transparency, interpretability, and trustworthiness of AI. It also exhibits higher data efficiency making it promising for edge deployments. Despite the algorithmic promises and demonstrations, unfortunately executing neurosymbolic workloads on current hardware (CPU/GPU/TPU) is challenging due to higher memory intensity, greater compute heterogeneity and access pattern irregularity, leading to severe hardware underutilization. This work proposes CogSys, a characterization and co-design framework dedicated to neurosymbolic AI system acceleration, aiming to win both reasoning efficiency and scalability. On the algorithm side, CogSys proposes an efficient factorization technique to alleviate compute and memory overhead. On the hardware side, CogSys proposes a scalable neurosymbolic architecture with reconfigurable neuro/symbolic processing elements (nsPE) and bubble streaming (BS) dataflow with spatial-temporal (ST) mapping for highly parallel and efficient neurosymbolic computation. On the system side, CogSys features an adaptive workload-aware scheduler (adSCH) to orchestrate heterogeneous kernels and enhance resource utilization. Evaluated across cognitive workloads, CogSys enables reconfigurable support for neural and symbolic kernels and exhibits >75x speedup over TPU-like systolic array with only <5% area overhead, as benchmarked under the TSMC 28nm technology node. CogSys achieves 4x-96x speedup compared to desktop and edge GPUs. For the first time, CogSys enables real-time abduction reasoning towards human fluid intelligence, requiring only 0.3 s per reasoning task with 4 mm2 area and 1.48 W power consumption.

==> Tables/algorithm_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
% \scriptsize
\centering
\caption{\textbf{\NAME Algorithm Optimization Performance.} \textnormal{Compared with NVSA, \NAME exhibits comparable reasoning capability with the proposed factorization and quantization. Neurosymbolic achieves higher cognitive accuracy than neuro-only methods.}}
% \vspace{0.05in}
\renewcommand*{\arraystretch}{1.3}
\setlength\tabcolsep{2.1pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|ccc|cc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dataset\\ Accuracy\end{tabular}} & \multicolumn{3}{c|}{Neurosymbolic Model}                                                                                                                                         & \multicolumn{2}{c|}{Non-neurosymbolic} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Human\\ \cite{raven}\end{tabular}}  \\ \cline{2-6}
                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NVSA\\ \cite{hersche2023neuro}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Algo Opt.)}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Quant.)}\end{tabular} & \multicolumn{1}{c|}{ResNet18}  & GPT-4  &                        \\ \hline
RAVEN~\cite{raven}                    & \multicolumn{1}{c|}{98.5\%} & \multicolumn{1}{c|}{$\text{98.7}_{\pm\text{0.3}}$\%}                                                            & $\text{98.6}_{\pm\text{0.4}}$\%                                                      & \multicolumn{1}{c|}{53.4\%}      & 89.0\%    & 84.4\%                   \\ \hline
I-RAVEN~\cite{iraven}                  & \multicolumn{1}{c|}{99.0\%}   & \multicolumn{1}{c|}{$\text{99.0}_{\pm\text{0.3}}$\%}                                                            & $\text{98.8}_{\pm\text{0.4}}$\%                                                    & \multicolumn{1}{c|}{40.3\%}      & 86.0\%    & 78.6\%                   \\ \hline
PGM~\cite{barrett2018measuring}                  & \multicolumn{1}{c|}{68.3\%}   & \multicolumn{1}{c|}{$\text{68.6}_{\pm\text{0.8}}$\%}                                                            & $\text{68.4}_{\pm\text{1.0}}$\%                                                    & \multicolumn{1}{c|}{36.8\%}      & 56.0\%    & N/A                   \\ \hline
\#Parameters                  & \multicolumn{1}{c|}{38~MB}   & \multicolumn{1}{c|}{32~MB}                                                            & 8~MB                                                    & \multicolumn{1}{c|}{42~MB}      & 1.7~TB    & N/A                   \\ \hline
\end{tabular}
}
\label{tab:eval_acc}
% \vspace{-5pt}
\end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t!]
% % \scriptsize
% \centering
% \caption{\textbf{\NAME Algorithm Optimization Performance.} \textnormal{Compared with NVSA, \NAME exhibits comparable reasoning capability with the proposed factorization and quantization. Neurosymbolic achieves higher cognitive accuracy than neuro-only methods.}}
% % \vspace{0.05in}
% \renewcommand*{\arraystretch}{1.3}
% \setlength\tabcolsep{2.1pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|ccc|cc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dataset\\ Accuracy\end{tabular}} & \multicolumn{3}{c|}{Neurosymbolic Model}                                                                                                                                         & \multicolumn{2}{c|}{Non-neurosymbolic} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Human\\ \cite{raven}\end{tabular}}  \\ \cline{2-6}
%                          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NVSA\\ \cite{hersche2023neuro}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Algo Opt.)}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Quant.)}\end{tabular} & \multicolumn{1}{c|}{ResNet18}  & GPT-4  &                        \\ \hline
% RAVEN~\cite{raven}                    & \multicolumn{1}{c|}{98.5\%} & \multicolumn{1}{c|}{98.7\%}                                                            & 98.6\%                                                      & \multicolumn{1}{c|}{53.4\%}      & 89.0\%    & 84.4\%                   \\ \hline
% I-RAVEN~\cite{iraven}                  & \multicolumn{1}{c|}{99.0\%}   & \multicolumn{1}{c|}{99.0\%}                                                            & 98.8\%                                                    & \multicolumn{1}{c|}{40.3\%}      & 86.0\%    & 78.6\%                   \\ \hline
% PGM~\cite{barrett2018measuring}                  & \multicolumn{1}{c|}{68.3\%}   & \multicolumn{1}{c|}{68.6\%}                                                            & $\text{68.4}_{\pm\text{1.0}}$\%                                                    & \multicolumn{1}{c|}{36.8\%}      & 56.0\%    & N/A                   \\ \hline
% \#Parameters                  & \multicolumn{1}{c|}{38~MB}   & \multicolumn{1}{c|}{32~MB}                                                            & 8~MB                                                    & \multicolumn{1}{c|}{42~MB}      & 1.7~TB    & N/A                   \\ \hline
% \end{tabular}
% }
% \label{tab:eval_acc}
% % \vspace{-5pt}
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t!]
% % \scriptsize
% \centering
% \caption{\textbf{\NAME Algorithm Optimization Performance.} \textnormal{Compared with NVSA, \NAME exhibits comparable reasoning capability with the proposed factorization and quantization. Neurosymbolic achieves higher cognitive accuracy than neuro-only methods.}}
% % \vspace{0.05in}
% \renewcommand*{\arraystretch}{1.3}
% \setlength\tabcolsep{2.1pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|ccc|cc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dataset\\ Accuracy\end{tabular}} & \multicolumn{3}{c|}{Neurosymbolic Model}                                                                                                                                         & \multicolumn{2}{c|}{Non-neurosymbolic} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Human\\ \cite{raven}\end{tabular}}  \\ \cline{2-6}
%                          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NVSA\\ \cite{hersche2023neuro}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Algo Opt.)}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{\NAME}\\ \textbf{(+Quant.)}\end{tabular} & \multicolumn{1}{c|}{ResNet18}  & GPT-4  &                        \\ \hline
% RAVEN~\cite{raven}                    & \multicolumn{1}{c|}{98.5\%} & \multicolumn{1}{c|}{98.7_{\rev{\pm0.4}\%}}                                                            & \rev{98.6_{\pm0.5}\%}                                                      & \multicolumn{1}{c|}{53.4\%}      & 89.0\%    & 84.4\%                   \\ \hline
% I-RAVEN~\cite{iraven}                  & \multicolumn{1}{c|}{99.0\%}   & \multicolumn{1}{c|}{99.0_{\rev{\pm0.3}\%}}                                                            & 98.8_{\rev{\pm0.4}}\%                                                    & \multicolumn{1}{c|}{40.3\%}      & 86.0\%    & 78.6\%                   \\ \hline
% PGM~\cite{barrett2018measuring}                  & \multicolumn{1}{c|}{68.3\%}   & \multicolumn{1}{c|}{68.7_{\rev{\pm0.8}}\%}                                                            & 68.4_{\rev{\pm1.0}}\%                                                    & \multicolumn{1}{c|}{36.8\%}      & 56.0\%    & N/A                   \\ \hline
% \#Parameters                  & \multicolumn{1}{c|}{38~MB}   & \multicolumn{1}{c|}{32~MB}                                                            & 8~MB                                                    & \multicolumn{1}{c|}{42~MB}      & 1.7~TB    & N/A                   \\ \hline
% \end{tabular}
% }
% \label{tab:eval_acc}
% % \vspace{-5pt}
% \end{table}


==> Tables/step_runtime.tex <==
\begin{figure}
% \vspace{-6pt}
\begin{minipage}[t!]{\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{Figs/Evaluation/step_runtime.pdf}
\end{minipage}% 
 \vspace{0.05in}
\begin{minipage}[b]{\columnwidth}
\tiny
\renewcommand*{\arraystretch}{1.2}
\setlength\tabcolsep{2.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
Steps & Jetson TX2 & Xavier NX & Xeon CPU & 2080Ti GPU & \textbf{\NAME (Ours)} \\ \hline
Step \circled{2}  & 61.2~sec.         & 38.6~sec.        & 12.8~sec.         & 3.5~sec.          & 0.086~sec.          \\ \hline
Step \circled{3}  & 112.5~sec.        & 80.9~sec.        & 33.4~sec.         & 5.7~sec.          & 0.057~sec.           \\ \hline
Step \circled{4}  & 6556.1~sec.       & 4074.7~sec.      & 1144.1~sec.       & 327.4~sec.        & 0.076~sec.           \\ \hline
Step \circled{5}  & 359.2~sec.        & 236.4~sec.       & 53.7~sec.         & 23.2~sec.         & 0.048~sec.          \\ \hline
\end{tabular}
}
\caption{\textbf{Step-by-Step Runtime Improvement}. \textnormal{\NAME significantly improves vector-symbolic operations (e.g., circular convolution) and GEMMs in heterogeneous neurosymbolic workloads, evaluated on 3$\times$3 RAVEN spatial-temporal reasoning task~\cite{raven}.}}
\label{fig:eval_step}
\vspace{-0.1in}
\end{minipage}
\end{figure}
